Empowering Counterfactual Reasoning over Graph Neural Networks through Inductivity

Graph neural networks (GNNs) have various practical applications, such as drug discovery, recommendation engines, and chip design. However, GNNs lack transparency as they cannot provide understandable explanations for their predictions. To address this issue, counterfactual reasoning is used. The main goal is to make minimal changes to the input graph of a GNN in order to alter its prediction. While several algorithms have been proposed for counterfactual explanations of GNNs, most of them have two main drawbacks. Firstly, they only consider edge deletions as perturbations. Secondly, the counterfactual explanation models are transductive, meaning they do not generalize to unseen data. In this study, we introduce an inductive algorithm called INDUCE, which overcomes these limitations. By conducting extensive experiments on several datasets, we demonstrate that incorporating edge additions leads to better counterfactual results compared to the existing methods. Moreover, the inductive modeling approach allows INDUCE to directly predict counterfactual perturbations without requiring instance-specific training. This results in significant computational speed improvements compared to baseline methods and enables scalable counterfactual analysis for GNNs.

==> 5_previous_work.tex <==

\section{Background - Perturbation based methods}
% \subsection{Background on GNNs}
\subsection{Interpretability of GNNs}
Interpretability of ML models is essential task and recently the interpretability of GNNs has gained a significant amount of attention. One of the early methods, GNNExplainer \cite{ying2019gnnexplainer} is a model-agnostic approach that provides interpretable explanations for predictions of any GNN-based model. Given a data (graph) instance, the method identifies a  subgraph structure as well as a small subset of node features that have significant impact in GNN’s prediction.  While GNNExplainer customizes the explanation for each instance, PGExplainer \cite{luo2020parameterized} attempts to have a global explanation for the GNN model. PGExplainer uses a deep learning approach to parameterize the explanation generation process. Since the neural network parameters are shared across the population of explained instances, it provides explanations for multiple instances collectively. It also has better generalization power because of its inductive setting.

Yan et al. \cite{yuan2021explainability} address the same problem of interpretabily on GNNs. For better explainability, their proposed method searches for important substructures/subgraphs of the input graph instead of finding nodes and edges that are important. It explores different subgraphs using Monte Carlo Search trees, and use approximation of Shapley values as importance score. Another model-agnostic framework \cite{lin2020graph} for interpreting important graph structure and node features combines an attention mechanism and sparsity regularization to yield an important subgraph and node feature subset. Li et al. \cite{li2020explain} formulate the explanation on weighted graph features used in GNN for node classification task. They consider weighted and directed graphs, and develop the graph neural network that uses both nodes and edges weights, where edge weights affect message aggregation.

In different domains such as NLP the interpretabilty of GNNs has been studied \cite{schlichtkrull2020interpreting}.  Schlichtkrull et al. \cite{schlichtkrull2020interpreting} have studied explainability of GNNs on two NLP tasks---question answering and semantic role labelling. 

\subsection{GNN Counterfactuals}

The interpretabilty of GNNs through counterfactual examples is relatively a new area of research. The paper that is most similar to our work also 
aims to find counterfactual explanations \cite{Cfgnnexplainer}. Counterfactual explanations are defined as the minimal perturbation to the input graph such that the prediction changes. The work only conisders edge deletions as graph perturbations and the proposed method gives approximately the minimum sized explanations, without having the explanation size as an input.

Other causal explanations involve an approach such as GEM \cite{lin2021generative} which explains GNNs on graph-structured data from a causal perspective. The proposed method is based on Granger Causality and has better generalization ability as it is unaware of the underlying GNN model. 

In chemistry, this work \cite{wellawatte2022model} deals with finding counterfactual graphs of molecules in a model agnostic fashion while adhering to relevant constraints such as maintaining the valency of atoms etc. unlike in \cite{Cfgnnexplainer}. \textbf{need to add: D. Numeroso and D. Bacciu, ArXiv, 2020.}

\subsection{To Include}

\begin{enumerate}
    \item \textbf{XGNN: Towards Model-Level Explanations of Graph Neural Networks (KDD 2020) (Should read this one)}
   

    \item \textbf{Causal Screening to Interpret Graph Neural Networks (OpenReview 2020)} 
    
    
    \item \textbf{Hard Masking for Explaining Graph Neural Networks (OpenReview 2020) - ZORRO}
    

    \item \textbf{Contrastive Graph Neural Network Explanation (ICML 2020)}
    
   % \item \textbf{Generative Causal Explanations for Graph Neural Networks(GEM) ICML 2021}
    
%    \item \textbf{CF-GNNExplainer AISTATS 2021}
    
    %\item \textbf{CFGNN-Explainer}: this has been added
    \item \textbf{CF-square}
    %\item \textbf{GEM}: this has been added - sourav
   
    
 
    
\end{enumerate}
